Swarm-Based Trajectory Generation and Optimization for Stress-Aligned 3D Printing

In this study, we present a novel swarm-based approach for generating optimized stress-aligned trajectories for 3D printing applications. The method utilizes swarming dynamics to simulate the motion of virtual agents along the stress produced in a loaded part. Agent trajectories are then used as print trajectories. With this approach, the complex global trajectory generation problem is subdivided into a set of sequential and computationally efficient quadratic programs. Through comprehensive evaluations in both simulation and experiments, we compare our method with state-of-the-art approaches. Our results highlight a remarkable improvement in computational efficiency, achieving a 115x faster computation speed than existing methods. This efficiency, combined with the possibility to tune the trajectories spacing to match the deposition process constraints, makes the potential integration of our approach into existing 3D printing processes seamless. Additionally, the open-hole tensile specimen produced on a conventional fused filament fabrication set-up with our algorithm achieve a notable ~10% improvement in specific modulus compared to existing trajectory optimization methods.

==> bibliographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author1.png}}]{Xavier Guidetti} received the B.S. and M.S. degrees in aerospace engineering from
the University of Virginia, Charlottesville, in 2001 and the Ph.D. degree in
mechanical engineering from Drexel University, Philadelphia, PA, in 2008.

From 2001 to 2004, he was a Research Assistant with the Princeton Plasma
Physics Laboratory. Since 2009, he has been an Assistant Professor with the
Mechanical Engineering Department, Texas A{\&}M University, College Station.
He is the author of three books, more than 150 articles, and more than 70
inventions. His research interests include high-pressure and high-density
nonthermal plasma discharge processes and applications, microscale plasma
discharges, discharges in liquids, spectroscopic diagnostics, plasma
propulsion, and innovation plasma applications. He is an Associate Editor of
the journal \emph{Earth, Moon, Planets}, and holds two patents.

Dr. Author was a recipient of the International Association of Geomagnetism
and Aeronomy Young Scientist Award for Excellence in 2008, and the IEEE
Electromagnetic Compatibility Society Best Symposium Paper Award in 2011.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author2.png}}]{Efe C. Balta} (M'76--SM'81--F'87) and all authors may include
biographies. Biographies are often not included in conference-related
papers. This author became a Member (M) of IEEE in 1976, a Senior
Member (SM) in 1981, and a Fellow (F) in 1987. The first paragraph may
contain a place and/or date of birth (list place, then date). Next,
the author's educational background is listed. The degrees should be
listed with type of degree in what field, which institution, city,
state, and country, and year the degree was earned. The author's major
field of study should be lower-cased.

The second paragraph uses the pronoun of the person (he or she) and not the
author's last name. It lists military and work experience, including summer
and fellowship jobs. Job titles are capitalized. The current job must have a
location; previous positions may be listed
without one. Information concerning previous publications may be included.
Try not to list more than three books or published articles. The format for
listing publishers of a book within the biography is: title of book
(publisher name, year) similar to a reference. Current and previous research
interests end the paragraph.

The third paragraph begins with the author's
title and last name (e.g., Dr.\ Smith, Prof.\ Jones, Mr.\ Kajor, Ms.\ Hunter).
List any memberships in professional societies other than the IEEE. Finally,
list any awards and work for IEEE committees and publications. If a
photograph is provided, it should be of good quality, and
professional-looking. Following are two examples of an author's biography.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author3.png}}]{John Lygeros} (M'87) received the B.S. degree in mechanical
engineering from National Chung Cheng University, Chiayi, Taiwan, in 2004
and the M.S. degree in mechanical engineering from National Tsing Hua
University, Hsinchu, Taiwan, in 2006. He is currently pursuing the Ph.D.
degree in mechanical engineering at Texas A{\&}M University, College
Station, TX, USA.

From 2008 to 2009, he was a Research Assistant with the Institute of
Physics, Academia Sinica, Tapei, Taiwan. His research interest includes the
development of surface processing and biological/medical treatment
techniques using nonthermal atmospheric pressure plasmas, fundamental study
of plasma sources, and fabrication of micro- or nanostructured surfaces.

Mr. Author's awards and honors include the Frew Fellowship (Australian
Academy of Science), the I. I. Rabi Prize (APS), the European Frequency and
Time Forum Award, the Carl Zeiss Research Award, the William F. Meggers
Award and the Adolph Lomb Medal (OSA).
\end{IEEEbiography}
